RECEIPT: REfine CoarsE-grained IndePendent Tasks for Parallel Tip decomposition of Bipartite Graphs

Tip decomposition is a crucial kernel for mining dense subgraphs in bipartite networks, with applications in spam detection, analysis of affiliation networks etc. It creates a hierarchy of vertex-induced subgraphs with varying densities determined by the participation of vertices in butterflies (2,2-bicliques). To build the hierarchy, existing algorithms iteratively follow a delete-update(peeling) process: deleting vertices with the minimum number of butterflies and correspondingly updating the butterfly count of their 2-hop neighbors. The need to explore 2-hop neighborhood renders tip-decomposition computationally very expensive. Furthermore, the inherent sequentiality in peeling only minimum butterfly vertices makes derived parallel algorithms prone to heavy synchronization. In this paper, we propose a novel parallel tip-decomposition algorithm -- REfine CoarsE-grained Independent Tasks (RECEIPT) that relaxes the peeling order restrictions by partitioning the vertices into multiple independent subsets that can be concurrently peeled. This enables RECEIPT to simultaneously achieve a high degree of parallelism and dramatic reduction in synchronizations. Further, RECEIPT employs a hybrid peeling strategy along with other optimizations that drastically reduce the amount of wedge exploration and execution time. We perform detailed experimental evaluation of RECEIPT on a shared-memory multicore server. It can process some of the largest publicly available bipartite datasets orders of magnitude faster than the state-of-the-art algorithms -- achieving up to 1100x and 64x reduction in the number of thread synchronizations and traversed wedges, respectively. Using 36 threads, RECEIPT can provide up to 17.1x self-relative speedup. Our implementation of RECEIPT is available at https://github.com/kartiklakhotia/RECEIPT.

==> rebuttal.tex <==
\section{Response to Reviewer Comments}
We thank the reviewers for providing insightful comments and pointing out areas of improvement in the paper. 
We first address the meta-review comments and then provide detailed response to the reviewers' comments along with  references to the corresponding edits (in blue) in the paper. Additionally, we had inadvertently excluded the amount of wedges traversed for vertex support initialization (one instance of butterfly counting) from the total wedge count for baseline \texttt{BUP}, in table~\ref{table:performance}. 
We have now corrected this discrepancy. The revised table shows that RECEIPT traverses less wedges than the baseline for all datasets (para 3 - sec.\ref{sec:baselines}). The code for RECEIPT is also made available at \url{https://github.com/kartiklakhotia/RECEIPT} (last para - abstract).

\subsection{Meta Review}\label{sec:meta}
\begin{enumerate}[leftmargin=*]
    \item \textbf{\underline{D1}: Provide more algorithmic details regarding the CD phase.}

    We have significantly updated the exposition of RECEIPT CD 
    (sec.\ref{sec:CD}) to address the issues raised by reviewers. First, we expand the details on tip number range computation and 
    adaptive determination (para 2 - sec.\ref{sec:CD}, and sec.\ref{sec:adaptive}). 
    
    Second, we elaborate on the choice of number of partitions $P$, both intuitively (paras 4,5 - sec.\ref{sec:receipt}) and empirically by design space exploration (para 6 - sec.\ref{sec:setup}). Please see responses to Reviewer 1 - \textbf{\underline{D1, D2}} (sec.\ref{sec:R1}) for more details.
    
    Lastly, we clarify that {\it some} of the butterflies in the original graph are {\it not} preserved in the subsets induced by CD. Hence, butterfly counting cannot be used in RECEIPT FD to initialize vertex 
    support in the induced subgraphs. However, we explain how the initial support values 
    required by RECEIPT FD are generated during RECEIPT CD and can be stored easily (para 
    5, 6 - sec.\ref{sec:receipt}, para 4 - sec.\ref{sec:CD}). Please see response to Reviewer 1 -
    \textbf{\underline{D4}} (sec.\ref{sec:R1}) for details. 
    
    \item\textbf{\underline{D2}: Provide more theoretical analysis where possible. Some feedback is 
    expected if it is difficult to make the theoretical analysis completed.}
 
    We have expanded the theoretical analysis and completed the proofs of correctness and complexity analysis. Specifically, we have included the following updates to address reviewer's concerns:
    \begin{itemize}
    \item We now explicitly show that all the butterflies with two vertices in the same vertex subset (say $U_i$) are preserved in the induced subgraph ($G_i$), and this is a sufficient condition to ensure correctness of support updates computed during peeling in RECEIPT FD (modified proof of theorem~\ref{theorem:receipt}). Using this argument, we prove the correctness of tip numbers outputted by RECEIPT. Please see response to Reviewer 1 - \textbf{\underline{D6, D4}} (sec.\ref{sec:R1}) for more details.
    \item We have included the complexity of computing scaling factor ($\mathcal{O}(n)$) and extracting minimum support vertices in RECEIPT FD ($\mathcal{O}(n\log{n})$) to our complexity analysis. Note that these updates do not alter the work-efficiency of RECEIPT.
    \item We have greatly simplified the proof of correctness of the partitioning (assigning vertices to tip number ranges) in RECEIPT CD (lemmas~\ref{lemma:parallel} and \ref{lemma:cd1}).
\end{itemize}
    %\klcomment{TODO}
    
    \item\textbf{\underline{D3}: Improve the presentation.}

    We have significantly improved the clarity of presentation. 
    \begin{itemize}[leftmargin=*]
        \item We have simplified the exposition in sections  \ref{sec:receipt} and \ref{sec:CD} to clarify important algorithmic
        details, especially regarding number of partitions and tip number range computation in RECEIPT CD (\textbf{\underline{D1}} -- sec.\ref{sec:meta}). We have made the overview of RECEIPT in sec.\ref{sec:receipt} more concise and highlighted important details for clarity. We have also improved the description of RECEIPT FD by explicitly highlighting the fundamental ideas inspired from the well known Longest Processing Time schedule rule (Reviewer 1 - \textbf{\underline{D3}} (sec.\ref{sec:R1})).
        \item We have incorporated major updates in the discussion and presentation of experiments (\textbf{\underline{D4}} -- sec.\ref{sec:meta}). We have also expanded the conceptual description of RECEIPT optimizations (Reviewer 3 - \textbf{\underline{D1}} (sec.\ref{sec:R3})).
        \item We have greatly simplified the proofs of correctness and improved the complexity analysis.
    \end{itemize}
    
    % \klcomment{Explanation of algorithms - Reviewer 1, \textbf{\underline{D1, D2, D6}} (sec.\ref{sec:R1} and Reviewer 2, \textbf{\underline{D4}} (sec.\ref{sec:R2}))}
    
    \item\textbf{\underline{D4}: Revise the experimental studies}
 
    We have thoroughly revised the experiments section to address the issues raised by
    the reviewers. First, we clarify the empirical contribution of different steps in RECEIPT.
    {\it The updated table~\ref{table:performance} now specifies the absolute 
    amount of wedge traversal and execution time incurred by butterfly 
    counting, used for vertex support initialization}. We also improve the explanation of observations reported in 
    figures \ref{fig:wb} and \ref{fig:tb} (para 3 - sec.\ref{sec:breakup}). Please see response to Reviewer 1 - \textbf{\underline{D8}} (sec.\ref{sec:R1}) for more details.
    
    Second, we improve the presentation and discussion of empirical benefits of workload optimizations. To effectively demonstrate the benefits of optimizations in figures \ref{fig:optWedges} and \ref{fig:optTime}, we plot the normalized values with respect to RECEIPT-- (RECEIPT without workload optimizations).
    We have also conceptualized a new metric (para 2 - sec.\ref{sec:optExp}) 
    derived from wedge traversal required for counting ($\wedge^{cnt}$) and 
    peeling ($\wedge^{peel}$). We use this metric to justify the observed 
    benefits of RECEIPT optimizations as shown in fig.\ref{fig:optWedges} and 
    \ref{fig:optTime}. Please see response to Reviewer 2 - \textbf{\underline{D1}} (sec.\ref{sec:R2}) for more details.
    
    Lastly, we provide detailed explanation of the scalability challenges and the differences between parallel speedup of tip decomposing $U$ and $V$
    vertex sets using RECEIPT (para 2 - sec.\ref{sec:scalability}). We have also updated fig.\ref{fig:scaleV} to have the same axis limits as fig.\ref{fig:scaleU} for ease of visual interpretation. Please see response to Reviewer 2 - \textbf{\underline{D3}} (sec.\ref{sec:R2}) for more details. 
    
    % \klcomment{Reviewer 1, \textbf{\underline{D8}} (sec.\ref{sec:R2}) and Reviewer 2, \textbf{\underline{D1, D2, D3}} (sec.\ref{sec:R3})}
\end{enumerate}

\subsection{Reviewer 1}\label{sec:R1}

\begin{enumerate}[leftmargin=*]
    \item \textbf{\underline{D1}: Section 3, Coarse-grained decomposition does the main job in the framework, however it is not clear how the authors determine the number of tip ranges/partitions.}
    
    We have updated the description of RECEIPT
    (para 3 - sec.~\ref{sec:receipt}) to specify that number of partitions $P$ is a user-defined parameter in our algorithm and influences the performance of different steps in RECEIPT (paras 4, 5 - sec.\ref{sec:receipt}). Intuitively, a large value of $P$ benefits RECEIPT FD but slows down RECEIPT CD and a small value of $P$ benefits RECEIPT CD while slowing down RECEIPT FD. We have revised the explanation in sec.~\ref{sec:setup} to provide these details underlying the choice of $P$.  For empirical evaluation, we perform a design space exploration over  
    the parameter $P$ to determine a suitable value (last para - sec.~\ref{sec:setup}, fig.\ref{fig:parts}). 
    Note that in all experiments (except the design space exploration itself), a uniform value of $P=150$ is used for all the datasets for fair 
    evaluation. While this may not be the optimum choice for every dataset, we show that it still significantly 
    outperforms the state-of-the-art.


    \item \textbf{\underline{D2}: Subsubsection 3.1.1, The range adaption works well for the cases where tip numbers are concentrated around
    a small intermediate range. However, when the tip numbers are contributed by large subgraphs, the scaling factor
    will break the subgraphs into smaller sets.}

    We have significantly revised the explanation of range adaptation (section~\ref{sec:adaptive}) to address the issue raised by the
    reviewer. 
    We have also expanded the description of range computation in Coarse-grained decomposition (para 2 - section~\ref{sec:CD}) to make the motivation behind range adaptation clearer. Specifically, we note that neither exact tip numbers nor the wedge counts of vertices in induced subgraphs are known prior to actual partitioning. We now make clear in the exposition how RECEIPT CD uses two proxies for range determination -- current vertex support as a proxy for tip numbers and wedge count in original graph as a proxy for wedge count in induced subgraph. 
    
    To balance the wedge counts of subsets, RECEIPT CD dynamically scales the target wedge coverage for $U_{i+1}$ with a scaling factor $s_i=\frac{tgt}{\sum_{u\in U_i}w[u]}\leq 1$, assuming that wedge coverage behavior of $U_{i+1}$ will be similar to $U_i$.
    Thus, when a large subgraph is encountered (say $U_i$ covers 
    significantly larger wedges than the average $tgt$), the target for \textit{immediately following} subset ($U_{i+1}$)
    is reduced. Note that $s_i$ only affects the target wedges of $U_{i+1}$. It has no impact on other subsets and is not used to break $U_i$ into smaller sets. Thus, a large subset $U_i$ may result in $U_{i+1}$ being small (covers less than average number of wedges), but it will not impact other subsets through $s_i$.
    Furthermore, if the target wedges for $U_{i+1}$ after applying the scaling factor $s_i$ is $tgt'$, then $tgt'$ is used to 
    compute $s_{i+1}$. Note that the wedge coverage here refers to wedges incident on vertices in original graph $G$, and not the induced subgraphs $G_i$.
    
    \item \textbf{\underline{D3}: Subsubsection 3.2.1, The proposed workload-aware-scheduling (WaS) is helpful for low number of threads.
However, when sufficient number of threads are available, the original order may yield better runtime than the WaS
without any sorting overhead. For example, suppose that T=3 in Figure 3, then the original order would finish at t=20
which is even better than WaS in this case.}

    We have updated sec.~\ref{sec:schedule} to address reviewer's concerns. 
    The workload aware scheduling is analogous to 
    Longest Processing Time (LPT) scheduling rule which is a known 
    $\frac{4}{3}$-approximation 
    algorithm.
    As pointed by the reviewer, this may not be an optimum strategy for any 
    arbitrary input but it exhibits a good approximation ratio.  Further, $P$ is very small ($<1000$) and hence, sorting overhead is negligible.
    
    Unlike LPT, the exact 
    processing times for peeling subsets in RECEIPT FD are unknown. Hence, we dynamically
    allocate subsets when threads get idle instead of computing an upfront mapping of subsets to threads. Further, we use the total wedge count of vertices $U_i$ in subgraph $G_i$, as a proxy for
    the execution time of $G_i$, to sort the subsets. 
    
    The graphical illustration given below (fig.\ref{fig:t3was}) shows the execution 
    times for a 3-thread system on the same example as fig.\ref{fig:schedule}. A dynamic 
    scheduler with tasks in original order will finish at $t=24$ whereas it will finish 
    at $t=20$ with workload aware scheduling. Note that subset IDs are popped from the 
    front of the task queue i.e. 
    \begin{enumerate}
        \item In workload aware scheduling, $U_4$ is scheduled first and $U_5$ is scheduled last.
        \item In original order scheduling, $U_1$ is scheduled first and $U_6$ is scheduled last.
    \end{enumerate}
    \begin{figure}[htbp]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/scheduling_t3.pdf}     
    \caption{Benefits of Workload-aware Scheduling (WaS) in a $3$-thread system.}
    \label{fig:t3was}
\end{figure}
 
 
    \item\textbf{\underline{D4}: Subsection 3.3, Can it be proven that all the butterflies in the original graph are preserved in the subsets
induced by CD? This is not a requirement, but it would be nice if it can be done.}

 We have updated the exposition (para 5, 6 - sec.\ref{sec:receipt})  and the proof of theorem~\ref{theorem:complexity} to clarify that {\it some} of the butterflies in the original graph are {\it not} preserved in the subgraphs induced on vertex subsets. Each butterfly has exactly two vertices in the set $U$ and two in set $V$. Only butterflies with two vertices in the same subset $U_i$ are preserved in the induced subgraphs (subgraph $G_i$ is induced on $U_i$ and $V$, and hence all the edges $(u,v)$ such that $u\in U_i$ are preserved in $G_i$ (proof for theorem~\ref{theorem:receipt})). We further show that this is a sufficient condition to guarantee correctness of support updates generated by peeling in RECEIPT FD (proof of theorem~\ref{theorem:receipt}).
 
 We also explicitly specify that because of the missing butterflies, per-vertex butterfly counting cannot be used in RECEIPT FD to initialize vertex support (para 5 - sec.\ref{sec:receipt}). However, we note that transient support values generated in RECEIPT CD can be used for initialization in RECEIPT FD and describe the mechanism to do so (para 6 - sec.\ref{sec:receipt}, para 4 - sec.\ref{sec:CD}). When $U_{i-1}$ is completely peeled in RECEIPT CD, the support of a vertex $u\in U$ reflects the number of butterflies it shares with vertices that are not yet peeled i.e. $\cup_{j\geq i}\{U_j\}$. This is precisely the value required to initialize the support of $U_i$ in RECEIPT FD. Hence, for all vertices $u\in U_i$, we store this value in $\bowtie^{init}_u$ during RECEIPT CD and use it in RECEIPT FD.
 
 
 \item\textbf{\underline{D5}: Subsection 3.3, It would be better if the authors mentioned the computational complexity for scaling factor is
o(1) since wedges of vertices are accumulated in the bins.}

We have updated the derivation of RECEIPT's work complexity (theorem~\ref{theorem:complexity} - sec.\ref{sec:analysis}) in accordance with the reviewer's recommendation.
% Computing scaling factor $s_i$ requires aggregating wedge count of vertices in $U_i$ which has a complexity of $\mathcal{O}\left(\abs{U_i}\right)$. For each subset, the scaling factor is computed once amounting to a total of $\mathcal{O}\left(\abs{U} \right) = \mathcal{O}\left(n\right)$ work done over all the subsets. Note that this does not alter the theoretical complexity of RECEIPT CD which is $\mathcal{O}\left(\sum_{u\in U}\sum_{v\in N_u}{d_v} + Pn\log{n}\right)$.

\item\textbf{\underline{D6}: Subsection 3.3, A theoretical analysis of the efficiency of RECEIPT vis a vis other parallel frameworks would be
good.}

To the best of our knowledge, P\textsc{ar}B\textsc{utterfly} is the only parallel framework for Tip Decomposition (excluding RECEIPT). We have updated section~\ref{sec:challenges} to state that P\textsc{ar}B\textsc{utterfly} is work-efficient with a complexity of $\mathcal{O}\left(\sum_{u\in U}\sum_{v\in N_u}{d_v} + \rho_v\log{m}^2\right)$ (as given in \cite{shiParbutterfly}), where $\rho_v$ is the number of peeling iterations. However, unlike RECEIPT, P\textsc{ar}B\textsc{utterfly} provides little speedup in practice over sequential implementation, as shown in table~\ref{table:performance}.

\item\textbf{\underline{D7}: The paper is dense and not easy to follow; it requires major re-writing. The analysis and poofs are not complete.
The experimental results are not well explained and in some parts they do not display promising contributions.}

We have significantly updated the presentation and exposition in the paper, especially 
regarding Coarse-grained Decomposition (sec.\ref{sec:receipt} and \ref{sec:CD}), to address
the concerns of the reviewer. We have made the overview of RECEIPT algorithm (sec.\ref{sec:receipt}) more concise
and highlighted important details for clarity.
As recommended by the reviewer, we have also completed the proofs of correctness and complexity analysis by showing the following:
\begin{itemize}[leftmargin=*]
    \item We now explicitly show that all the butterflies with both vertices in the same subset (say $U_i$) are preserved in the induced subgraph ($G_i$). We further prove that this is a sufficient condition to ensure correctness of RECEIPT (\textbf{\underline{D4}}).
    \item We have revised the proof of theorem~\ref{theorem:receipt} to show that when peeling a subset $U_i$, for both RECEIPT FD and BUP,
    \begin{enumerate*}
    \item initial vertex supports are same,
    \item peeling a vertex generates same updates for every vertex in $U_i$, and
    \item vertices are peeled in the same order.
    \end{enumerate*}
    Thus, we show that the tip number outputted by RECEIPT FD is the same as BUP (known to be correct~\cite{sariyuce2016peelingarxiv}).
    \item We have updated the complexity analysis to incorporate the work done in computing scaling factor ($\mathcal{O}(n)$) and extracting minimum support vertices in RECEIPT FD ($\mathcal{O}(n\log{n})$). Note that these contributions do not alter the overall complexity of RECEIPT. 
\end{itemize}
In addition, we have simplified the proof of correctness of the partitioning (assigning vertices to tip number ranges) in RECEIPT CD (lemmas~\ref{lemma:parallel} and \ref{lemma:cd1}).

We have also revised the experiments section (figures \ref{fig:optTime} and \ref{fig:optWedges}, sections \ref{sec:optExp} and \ref{sec:breakup}) to provide a better explanation of the behavior of RECEIPT and its optimizations. Please see responses to \textbf{\underline{D8}} (sec.\ref{sec:R1}), and Reviewer 2 - \textbf{\underline{D1, D3}} (sec.\ref{sec:R2}) for more details.


\item\textbf{\underline{D8}: The execution time of the algorithms especially pvBcnt() is highly affected by the density of the graph. However,
density of datasets are not mentioned. As suggested by the number of vertices and edges provided in Table 2, the
density of graph datasets are low. On the other hand, the datasets have billions of wedges. Yet high number of
wedges does not necessarily imply high wedge per vertex. In section 5.2.2, the authors mention that the distribution
of wedges are skewed in datasets, however it would have been clearer if the authors reported the skewness of
distribution for the datasets as well as the average vertex degrees and graph density. This information can also
explain figures 8 and 9 in section 5.2.3. For instance the Tr dataset apparently is sparsest dataset which in turn has
the smallest execution time for pvBcnt().}

RECEIPT uses the butterfly counting algorithm of Wang et al.\cite{wangButterfly}. As given in \cite{wangButterfly}, the execution time of counting (pvBcnt) is determined by the quantity $\sum_{\left(u,v\right)\in E}{\min{\left(d_u, d_v\right)}}$. To make the contribution of counting clearer, we now explicitly specify the amount of wedge traversal and execution time of pvBcnt (updated table~\ref{table:performance}) and report the average degree of datasets (updated table~\ref{table:datasets}). Wang et al.\cite{wangButterfly} show that the counting algorithm 
only traverses wedges in which degree of the middle vertex is lower than the degree of the 
end vertex (revised sec.\ref{sec:counting}). Consequently, any edge can appear in $\mathcal{O}\left(\min{\left(d_u, d_v\right)}\right)$ 
wedges traversed during counting. 


Using the newly reported wedge traversal of counting, we further conceptualize a new ratio $r=\frac{\wedge^{peel}}{\wedge^{cnt}}$, where $\wedge^{peel}$ and $\wedge^{cnt}$ denote the 
number of wedges traversed for peeling all vertices in $U$ ($\wedge^{BUP}-\wedge^{pvBcnt}$ in table~\ref{table:performance}) and for butterfly counting 
($\wedge^{pvBcnt}$ in table~\ref{table:performance}), respectively. 
Datasets with large value of $r$ (for example \textit{ItU, LjU, EnU} and \textit{TrU} with $r>1000$) benefit heavily from HUC optimization. Especially for \textit{TrU} ($r>33,500$), HUC enables \textbf{$57\times$} and \textbf{$42\times$} reduction in wedge traversal and execution time, respectively. We have updated section~\ref{sec:optExp} to include this explanation and make it clearer for the reader. This ratio $r$ better explains the observed benefits of HUC optimization compared to wedge distribution, because decision making in HUC depends only on total wedge count of vertices peeled in an iteration, and not on how they are distributed across the vertices.



% Large datasets such as \textit{ItU, LjU, EnU} and \textit{TrU} exhibit high value of $r$($>1000$). In such cases, HUC often replaces peeling by a re-count, thereby dramatically 
% reducing the workload and the execution time. 

The reported statistics of pvBcnt in revised table~\ref{table:performance} also explain the results in figures~\ref{fig:wb} and \ref{fig:tb} (updated para 3 - sec.\ref{sec:breakup}). Tip decomposition of \textit{TrU} and \textit{TrV} datasets traverses a large amount of wedges and exhibit high execution time (table~\ref{table:performance}). As a result, the percentage contribution of \texttt{pvBcnt} (relative to RECEIPT's total) is very small even though the absolute time and wedge traversal for butterfly counting in \textit{Tru/TrV} is larger than all datasets except \textit{DeU/DeV} and \textit{OrU/OrV}.

\end{enumerate}

\subsection{Reviewer 2}\label{sec:R2}

\begin{enumerate}[leftmargin=*]
\item\textbf{\underline{D1}: Improve figure 7 and the discussion of the results for the two proposed optimizations.}

We have updated the fig.\ref{fig:optWedges} and \ref{fig:optTime} and the exposition regarding the same (para 2 - sec.\ref{sec:optExp}) as per reviewer's comments. Both the figures are now plotted on linear scale with wedges and execution time normalized to RECEIPT-{}-. Using $TrU$ as an example dataset, we now emphasize that for some of the graphs, the workload reduction optimizations provide significantly large speedup.

HUC reduces wedge traversal by opting to re-count butterflies instead of peeling in 
selective iterations. To better understand the impact of HUC, we define a ratio $r$ that 
quantifies the relative work required for peeling all vertices vs counting all butterflies.
Specifically, $r=\frac{\wedge^{peel}}{\wedge^{cnt}}$, where $\wedge^{peel}$ and $\wedge^{cnt}$ indicate the 
number of wedges traversed for peeling all vertices in $U$ ($\wedge^{BUP}-\wedge^{pvBcnt}$ in table~\ref{table:performance}) and for butterfly counting 
($\wedge^{pvBcnt}$ in table~\ref{table:performance}), respectively. 
Datasets with large value of $r$ (for example \textit{ItU, LjU, EnU} and \textit{TrU} with $r>1000$) benefit heavily from HUC optimization. In these datasets, peeling is replaced by a re-count in several high workload iterations, thereby dramatically reducing the wedges traversed. Especially for \textit{TrU} ($r>33,500$), HUC enables \textbf{$57\times$} and \textbf{$42\times$} reduction in wedge traversal and execution time, respectively. Contrarily, in datasets with small value of $r$ (\textit{ItV, DeV, OrV, LjV and EnV} with $r<5$ due to low $\wedge^{peel}$), none of the iterations utilize re-counting. Consequently, performance of RECEIPT- and RECEIPT-{}- is similar for these datasets.

\item\textbf{\underline{D2}: Discuss/Explain/Argument why RECEIPT-- works better on some graphs than RECEIPT-. Why this happens? Does it depend on the characteristics of the underlying graph? What are these characteristics?}

Please see the response to \textbf{\underline{D1}}.

\item\textbf{\underline{D3}: Fix Y-Axis of Figure 11 and discuss it. Why when peeling set V, the scalability is worse?}

We have fixed the fig.\ref{fig:scaleV} as per reviewer's suggestion. We provide detailed explanation of differing scalability for peeling $U$ and $V$ sets (para 2 - sec.\ref{sec:scalability}). RECEIPT CD is likely to exhibit lower parallel speedup for peeling $V$ set due to its lower wedge workload compared to $U$ set (by definition, para 3 - sec.\ref{sec:setup}). Hence, RECEIPT CD traverses a small amount of wedges between successive synchronization rounds which in turn, increases the relative overheads of parallelization. Note that a synchronization round represents a peeling iteration and threads actually synchronize multiple (but constant) times within each iteration (para 1 - sec.\ref{sec:baselines}).
% . It can also render RECEIPT CD prone to load imbalance. With fewer wedges per iteration, it is challenging for OpenMP dynamic scheduing to balance thread workload if the distribution of vertex wedge counts is skewed. 
This affects the parallel speedup of RECEIPT CD and in turn, RECEIPT overall as this is the highest workload step.

The parallel speedup is especially poor for \textit{ItV} because it is a very small dataset that gets peeled in $<4$s and requires very little computation ($0.56$B wedges). Hence, employing a large number of threads is not useful as the parallelization overheads and initialization of (per-thread) data structures dominates the overall execution.

We have also included a detailed discussion on scalability challenges of RECEIPT FD (para 3 - sec.\ref{sec:scalability}). However, we note that RECEIPT FD contributes $<25\%$ of the total execution time for almost all datasets (fig.\ref{fig:tb}, para 3 - sec.\ref{sec:breakup}). We are also investigating finer granularity task creation to alleviate potential load imbalance due to non-uniform vertex wedge counts in peeling iterations of RECEIPT CD (bullet point 3, sec.\ref{sec:extensions}).
% \kldelete{
% Load imbalance in RECEIPT FD - primarily arises due to varying wedge workload in the subgraphs induced on vertex subests. This is because the partitioning in RECEIPT
% CD takes into consideration wedge counts of vertices in original
% graph $G$, whereas actual work in RECEIPT FD is determined
% by wedges within induced subgraphs. The load imbalance combined with the
% overheads of generating induced subgraphs and applying 
% support updates to heap structure (instead of array in 
% RECEIPT CD) explains why the contribution of RECEIPT FD to
% execution time (fig.\ref{fig:tb}) is greater than its 
% contribution to wedge workload (fig.\ref{fig:wb}). Yet, RECEIPT FD contributes $<25\%$ to the overall execution time in almost all datasets.}

\item \textbf{\underline{D4}: Fix other minor issues}
\begin{itemize}[leftmargin=*]
    \item \textbf{The authors claim: "Note that the parallel bucketing structure of Julienne is not work-efficient in the context of tip decomposition", but they do not explain why. It would be great if the authors could extend on this.}
    
    We borrow this claim from the paper that describes P\textsc{ar}B\textsc{utterfly} framework~\cite{shiParbutterfly}. 
    Due to the work-inefficiency of Julienne's bucketing, the authors of \cite{shiParbutterfly} derive
    computational complexity of P\textsc{ar}B\textsc{utterfly} assuming a parallel fibonacci heap structure for finding minimum support vertices, even though their implementation uses Julienne for practical reasons.
    
    As per our discussion with the authors of Julienne and 
    P\textsc{ar}B\textsc{utterfly}, the problem arises when
    searching for the next non-empty bucket with minimum 
    support value. Julienne has to iterate over empty 
    buckets created due to transient support value of 
    vertices, performing logarithmic work per bucket. In
    the worst case, Julienne may materialize $\theta^{max}$
    buckets as the transient vertex support values may 
    range from $0$ to $\theta^{max}$. This will lead to an 
    additional $\mathcal{O}\left(\theta^{max}\log{n}\right)
    $ term in the complexity making it work-efficient.
    Note that there are at most $\abs{U}$ unique tip number
    values. Hence, at most $\abs{U}$ buckets will be 
    non-empty from which minimum support vertices are 
    extracted for peeling. The same reasoning would apply to RECEIPT CD 
    if Julienne's bucketing structure were to be used.

    However, since we do not use Julienne's bucketing structure in
    our theoretical analysis or actual implementation (we only 
    use array in RECEIPT CD and sequential min-heap data structure in
    RECEIPT FD), we have revised section \ref{sec:CD} and removed this 
    claim. 
    %Hence, explicit discussion of 
    %theoretical complexity of assuming the use of Julienne's parallel bucketing 
    %might be confusing to the reader.
    
    \item \textbf{Presentation issues on page 7, lemma \ref{lemma:parallel} (abbreviation "wlog") and page 9, section \ref{sec:results}.}
    We have fixed these presentation issues in accordance with reviewer's comments. We have also removed typographical errors after a careful proofread.
\end{itemize}


\subsection{Reviewer 3}\label{sec:R3}
\begin{enumerate}[leftmargin=*]
    \item \textbf{\underline{D1}: Some further analysis on the optimization techniques.}
    We have significantly expanded both conceptual 
    (sec.\ref{sec:optimizations}) and empirical (sec.\ref{sec:optExp}) 
    analysis of the optimizations. We formalize the costs of peeling a 
    specific set of vertices vs re-counting butterflies for all vertices, 
    which is used for decision making in HUC (para 2 - sec.\ref{sec:optimizations}). 
    We have incorporated new insights into the empirical benefits of 
    optimizations (sec.\ref{sec:optimizations}). To explain the observations in figures \ref{fig:optWedges} and \ref{fig:optTime}, we conceptualize a ratio $r=\frac{\wedge^{peel}}{\wedge^{cnt}}$, where $\wedge^{peel}$ and $\wedge^{cnt}$ indicate the 
number of wedges traversed for peeling all vertices in $U$ and for butterfly counting, respectively. Please see Reviewer 2 - \textbf{\underline{D1}} (sec.\ref{sec:R2}) for more details. 

    \item \textbf{\underline{D2}: Some further discussion on distributed setting.}
    We have updated para 2 - sec.\ref{sec:extensions}, that discusses distributed-memory tip decomposition. Owing to the high computational complexity of tip decomposition, this is a natural direction for future work that we are investigating. We believe that the fundamental concepts underlying RECEIPT can be utilized in designing distributed algorithms as well. We 
    have revised sec.\ref{sec:extensions} to include a commentary on the 
    importance and challenges of distributed tip decomposition. Note that currently, RECEIPT is implemented for shared-memory multicore servers.  
    
\end{enumerate}

\end{enumerate}
